Set Similarity Search for Skewed Data

Set similarity join, as well as the corresponding indexing problem set similarity search, are fundamental primitives for managing noisy or uncertain data. For example, these primitives can be used in data cleaning to identify different representations of the same object. In many cases one can represent an object as a sparse 0-1 vector, or equivalently as the set of nonzero entries in such a vector. A set similarity join can then be used to identify those pairs that have an exceptionally large dot product (or intersection, when viewed as sets). We choose to focus on identifying vectors with large Pearson correlation, but results extend to other similarity measures. In particular, we consider the indexing problem of identifying correlated vectors in a set S of vectors sampled from {0,1}^d. Given a query vector y and a parameter alpha in (0,1), we need to search for an alpha-correlated vector x in a data structure representing the vectors of S. This kind of similarity search has been intensely studied in worst-case (non-random data) settings. Existing theoretically well-founded methods for set similarity search are often inferior to heuristics that take advantage of skew in the data distribution, i.e., widely differing frequencies of 1s across the d dimensions. The main contribution of this paper is to analyze the set similarity problem under a random data model that reflects the kind of skewed data distributions seen in practice, allowing theoretical results much stronger than what is possible in worst-case settings. Our indexing data structure is a recursive, data-dependent partitioning of vectors inspired by recent advances in set similarity search. Previous data-dependent methods do not seem to allow us to exploit skew in item frequencies, so we believe that our work sheds further light on the power of data dependence.

==> correlated.tex <==
\section{Pearson Correlation Math}

In this section we discuss how the probabilities work under the situation where 
each element $y$ is generated from a distribution $D$.  
Each query $q$ is $\rho$-correlated with a particular element $x$.

So far in our analysis, we have assumed that $D$ sets bits independently; in particular, bit $i$ is set with probability $p_i$.  
(We'll call that $w_i$ here for clarity.)
Here, we calculate the probability that the $i$th bit is set in both $x$ and $q$ ($p^{11}_i$), that it is set in neither ($p^{00}_i$), or it is only set in one ($p^{01}_i$ and $p^{10}_i$).  

We set up a system of equations.  Clearly, one of the above must happen, so
\[
    p^{11}_i +p^{10}_i+ p^{01}_i+ p^{00}_i = 1
\]

We want bit $i$ of both $x$ and $q$ to be set with probability $w_i$, so 
\begin{align*}
    p^{01}_i+ p^{11}_i  = w_i\\
    p^{10}_i+ p^{11}_i  = w_i
\end{align*}

Finally, the Pearson correlation coefficient ($\rho$, which we'll overload in this section) between variables $X$ and $Y$ is defined as 
\[
    \rho = \E\left[ \frac{(X - \E[X])(Y - \E[Y])}{\sigma_x\sigma_y}\right]
\]

Since 
$\sigma_x\sigma_y = w_i(1-w_i)$, we can take the above cases over all four of $p^{11}_i$, etc., to get 
\[
    \rho = p^{00}_i  \frac{w_i}{1-w_i} - p^{01}_i - p^{10}_i + p^{11}_i\frac{1-w_i}{w_i}.
\]

We have four equations and four variables; we can begin solving.

First, we reduce to two equations in two variables.  Adding the second and third equations and subtracting the first,
\[
    p^{10}_i + p^{01}_i = 2 - 2w_i - 2p^{00}_i.
\]

Substituting into the fourth,
\begin{align}
\rho = p^{00}_i  \frac{w_i}{1-w_i} -2 + 2w_i + 2p^{00}_i  + p^{11}_i\frac{1-w_i}{w_i}.
\end{align}

We obtain the second equation similarly.  Taking the first equation, and subtracting the second and third, 
\begin{align}
    p^{11}_i - p^{00}_i = 2w_i - 1
\end{align}

We now solve for $p^{11}_i$ using the above.  Substituting, we immediately obtain
\[
    \rho = p^{00}_i  \frac{w_i}{1-w_i} -2 + 2w_i + 2p^{00}_i  + (2w_i - 1 + p^{00}_i)\frac{1-w_i}{w_i}.
\]

Everything cancels nicely, and
\[
    \rho = \frac{p^{00}_i}{w_i(1-w_i)} - \frac{1 - w_i}{w_i},
\]
so $ p^{00}_i = \rho w_i(1-w_i) + (1-w_i)^2$.   Substituting, 
$ p^{11}_i = \rho w_i(1-w_i) + w_i^2$.

Finally, $ p^{01}_i = w_i - p^{11}_i$.


\subsubsection*{Generating $q$}

Given an element $x$, we want to generate $q$.  Consider the $i$th bit of $x$.  First, assume $x_i = 1$.  Then $q_i = 1$ with probability $p_{11}/w_i = \rho(1-w_i) + w_i$; taking the complement, $q_i = 0$ with probability $(1-\rho)(1-w_i)$.

Similarly, assume $x_i = 0$.  Then $q_i = 0$ with probability $\rho w_i + (1-w_i)$, and $q_i = 1$ with probability $w_i(1-\rho)$.


%\subsection{Applying To Chosen Path}
%
%\subsubsection*{Distances}
%
%For now, we assume concentration bounds (for example, we assume that the Hamming weight of all $y$ is exactly its expectation).  This should be relaxed or proven in the future.
%
%The expected similarity to a far point is given by (since $q$ and every far point have their digits set independently)
%\[
%    b_2 = \frac{\sum_i w_i^2}{\sum_i w_i}.
%\]
%
%The expected similarity to a close point is given by
%\[
%    b_1 = \frac{ \sum_i \rho w_i(1-w_i) + w_i^2}{\sum_i w_i} = b_2 + \rho\frac{\sum_i w_i(1-w_i)}{\sum_i w_i}
%\]
%
%%If enough $w_i$ are sufficiently small, we have $b_1\approx b_2 + \rho$.
%
%This can also be written as 
%\[
%    b_1 = \rho + (1-\rho)\frac{\sum w_i^2}{\sum w_i}
%\]
%
%
%\subsubsection*{Conditional Probability}
%An important quantity for chosen path is 
%\begin{align*}
%\hat{p}_i = \Pr(x_i = 1 ~|~ q_i = 1) &= \frac{p^{11}_i}{p^{01}_i + p^{11}_i}\\
%    &= \rho(1-w_i) + w_i\\
%    &= w_i(1-\rho) + \rho
%\end{align*}
%
%Following the lead of Chosen Path, 
%we may want to sample with probability $\frac{1}{\hat{p}_i q}$.  First, we must check if this is $< 1$.  We have that $\rho > 1/q$ (otherwise the close/correlated point $x$ has only a single digit more in common with $q$ than a random far point, making our search hopeless); since $\hat{p}_i > \rho$ we are done.
%
%If $w_i$ is very small, we have $\hat{p}_i \approx \rho$.  Thus, all digits are sampled with approximately the same probability, leading to (essentially) chosen path.
%
%If $w_i$ is not as small, we may have $\hat{p}_i > \rho$, or even $\hat{p_i} \approx w_i$ (if $\rho$ is small compared to $w_i$).  However, it seems likely that we should ignore these points.  After all, if $\hat{p_i}\approx w_i$, then for a far point $y$ and the close point $x$, $\Pr(y_i = 1) = w_i \approx \Pr(x_i = 1)$.
%
%\subsubsection*{Number of digits to keep in a filter}
%
%Using the same analysis as in original Chosen Path, we have
%\[
%    \E[|F^k(q)|] = \left(\sum_i \frac{1}{q(\rho + w_i(1-\rho))} \right)^k
%\]
%and 
%\[
%    \E[\text{number of elements in all filters of $q$}] = n \left(\sum_i \frac{w_i}{q(\rho + w_i(1-\rho))} \right)^k
%\]
%
%Solving, we obtain
%\[
%    k = \frac{\log n}{\log \frac{\sum_i 1/(\rho + w_i(1-\rho))}{\sum_i w_i/(\rho + w_i(1-\rho)) }}
%\]


==> estimatingrho.tex <==

\section{Estimating $\rho^*$}
\subsection{Upper bounds on $\rho*$}
Let $0\leq p_1,p_2,\ldots, p_q\leq 1$, let $q\in \mathbb{N}$, and let $0<b_1<1$ be given. Assume that $\sum_{j=1}^q p_j\leq b_1q$. We seek the solution, $\rho^*$, to the equation
\[
\sum_{j=1}^q p_j^\rho = b_1q,
\]
where $0\leq \rho\leq 1$. Taking logs and rearranging yields the equivalent equation  
\begin{equation}
\log\left(\sum_{j=1}^q p_j^\rho\right)-\log(b_1q)=0.
\label{eq:rho}
\end{equation}
Define $f:[0,1]\rightarrow\mathbb{R}$ by
\[
f(\rho)=\log\left(\sum_{j=1}^q p_j^\rho\right) - \log(b_1q).
\]
Note that $\sum_{j=1}^q p_j^\rho$ is a positive linear combination of log-convex functions and hence log-convex. 
It follows that $f$ is convex. In fact, $f$ is strictly convex unless all $p_j$'s are identical. 
Also, $f$ is strictly decreasing. Furthermore, $f(0)=\log(1/b_1)$ while $f(1)=\log(\sum_{j=1}^q p_j) - \log(b_1q)$ and, by assumption on $b_1$, this implies that $f(0)>0>f(1)$. 

For $0\leq c \leq 1$, define $g_c(\rho)=f(0)+\rho\frac{f(c)-f(0)}{c}$, i.e., $g$ is the line segment between $(0,f(0))$ and $(c,f(c))$.
Since $f$ is convex, $f(\rho)\leq g_c(\rho)$ for $\rho\in [0,c]$. 
Combined with the fact that $f$ is decreasing, this means that if $g_c$ is zero for some $\rho\in [0,c]$, then the zero of $g_c$ is an upper bound on $\rho^*$. 
As a consequence, whenever we have some (non-tight) upper bound, $c$, on $\rho^*$, we can obtain a better upper bound by solving $g_c(\rho)=0$. 
Now, $g_c(\rho)=0$ if $\rho=-cf(0)/(f(c)-f(0))$. This proves that
\begin{equation}
\rho^*\leq c \Rightarrow \rho^*\leq \frac{\log(b_1)}{\frac{1}{c}\log\left(\sum_{j=1}^q p_j^c/q\right)}.
\label{eq:recursiverho}
\end{equation}
In particular, using the trivial upper bound on $\rho^*$ of $c=1$, we get
\[
\rho^*\leq \frac{\log(b_1)}{\log\left(\sum_{j=1}^q p_j/q\right)}.
\]
Here, equality holds if and only if all $p_j$'s are equal (in which case the upper bound reduces to $\log(b_1)/\log(p)$ where $p_j=p$ for all $j$). In all other cases, $f$ is strictly convex and hence $p^*$ is strictly smaller than the expression on the right-hand side.

Note that as a consequence of (\ref{eq:recursiverho}), if we define $\rho_1=1$ and $\rho_{i+1}=-\rho_if(0)/(f(\rho_i)-f(0))$, we get a infinite sequence such that $\rho_i\rightarrow \rho^*$ from above as $i\rightarrow\infty$.

\subsection{Exact computation in specific cases}
One of the few cases where eq. (\ref{eq:rho}) can be solved analytically is when the $p_j\in\{p_a,p_b\}$ and $p_b=p_a^2$. In this case, the equation reduces to
\[
q_a p_a^\rho + q_b (p_a^\rho)^2 = b_1q.
\]
It follows that $p_a^\rho=\frac{\sqrt{4q_b b_1q+q_a^2}-q_a}{2q_b}$.
\subsection{Lower bounds on $\rho^*$}
Since $f$ is convex and smooth, a first-order Taylor approximation yields $f(0)+\rho f'(0)\leq f(\rho)$. Thus,
\[
\rho^*\geq \frac{-f(0)}{f'(0)}=\frac{\log(b_1)}{\sum_{j=1}^q \log(p_j)/q}.
\]
Note that if $p_j=p$ for all $j$, this lower bound reduces to $\log(b_1)/\log(p)$.



